Toward a language-theoretic foundation for planning and filtering

We address problems underlying the algorithmic question of automating the co-design of robot hardware in tandem with its apposite software. Specifically, we consider the impact that degradations of a robot's sensor and actuation suites may have on the ability of that robot to complete its tasks. We introduce a new formal structure that generalizes and consolidates a variety of well-known structures including many forms of plans, planning problems, and filters, into a single data structure called a procrustean graph, and give these graph structures semantics in terms of ideas based in formal language theory. We describe a collection of operations on procrustean graphs (both semantics-preserving and semantics-mutating), and show how a family of questions about the destructiveness of a change to the robot hardware can be answered by applying these operations. We also highlight the connections between this new approach and existing threads of research, including combinatorial filtering, Erdmann's strategy complexes, and hybrid automata.

==> omit.tex <==

This kind of groundwork is important because we believe that the lack of any
such theory has hampered progress in robotics to date.

% A challenging and basic problem in all scientific and engineering enterprises
% is that of determining the right models for, and abstractions of, the thing
% being studied. It is likely that this challenge is a key factor in the current
% gap between robotics science and robotics systems.  If we consider the former
% to be comprised primarily of theoretical constructs and the latter of physical
% demonstrations, though we admit this to be a slight caricature, then the
% fundamental and foundational challenge is that we have difficulty assessing the
% faithfulness of a particular model for some part of a physical robot system.
% So far, a notion of faithfulness that generalizes widely, say across robots and
% environments, has proved elusive.  We are fully aware that our caricature omits
% detail: omission and control of detail is, in a very real sense,
% the topic of this paper.


% Interesting questions arise when one considers how modifications to a given
% robot's capabilities alter the planning and estimation efforts that robot must
% undertake.
%
% This paper develops theoretical tools that we believe to be helpful
% for thinking about such aspects.

%Our current shallow understanding of the relationship between sensor
%idealizations and their hardware realizations is highlighted in practical work,
%such as \citep{vaughan03}.  That work, later developments, and open-source
%efforts generally, have provided interfaces for several classes of device.  Our
%work is an initial\,---but by no means complete---\,exploration of how one
%might provide theoretical underpinnings for current software efforts.  Rather
%than clustering existing hardware devices from the bottom up, this paper
%explores device abstractions from the top downward, defining an abstract
%idealization and general operations thereon to represent and analyze the
%shortcomings and fallibility of particular hardware instantiations. 

% Compare, for example, to other areas in computing research,
% where algorithmic results are established for settings that, after a
% critical-mass and a flurry of effort, become standardized.  With some notable
% exceptions, the field of robotics has few comparable cases.
% Motion planning is a notable exception---arguably, the attention given
% to the problem is not a consequence of the problem being
% important\footnote{Patently, it is not important: the information required to
% solve the problem as typically posed is seldom available.} so much as it
% becoming a standardized and crisply formulated problem.


%% Such questions include: {\sl 
%% Is task $T$ feasible with sensor $S$?
%% If actuator $A$ degrades to $A'$ will that affect task feasibility? If the degradation is gradual is there a precise, theoretical cut-off point in functionality?
%% Supposing that cost savings of \$200 are to be made by using cheaper sensors and actuators, should 
%% all the saving be made in actuators? Or all sensors? Or is there a point at which having better
%% actuators is useless for certain sensors, or can they compensate?}
%% These foundational questions bear on many aspects of robotics and a
%% means for answering them is important in making informed design
%% decisions\,---especially when selecting sensors, actuators, and computational
%% resources.

%%%% Comment: This is an important idea that seems not to fit in this paper -- we
%%%% don't have and complexity results or hardness bounds.
%% A large element of the appeal of the approach is that it enables hardness
%% results and complexity bounds, giving a sense of the feasibility of such design
%% decisions.

In this paper, we address the problem of determining whether certain
perturbations in sensor specification or performance affect the behavior of a
robotic system. (Figure~\ref{fig:idealtorealviamaps} provides a visual overview.)
%
We seek to understand
  which changes to a sensor suite might make a system inoperable,
  which changes result in graceful degradation of performance, and
  which changes might have little or no effect.
Transformations that, in the picture, represent hardware realizations of the
ideal range sensor may either preserve behavior or alter it. In that latter
case, we say it is destructive.  The key insight\,---an insight not unique to
this paper, but one whose long history is briefly reviewed in
Section~\ref{sec:related_work}---\,is that whether a transformation is
destructive or not depends on the information needed for the task being
performed.



Thus far, other than the potentially infinite action- and observation-alphabets
and their specific alternating structure, the definitions are close to classic
formal language theory.  The set of executions on $G$ are taken to comprise
$L(G)$, the language induced by p-graph $G$.  Also, since $\Vinit(G) \subseteq
V(G)$, the language of every p-graph includes the empty sequence. 


%
% NOTE:  pigeonhole principle appears to useful in showing that to every non-homomorphic
%                       there is some homomorphic that is no-longer. (strictly shorter?)
%           rephrasing attempt: for any (W, \Vgoal), and g \in Vgoal, the shortest 
%                               execution arriving at $g$ is produced by some 
%                               homomorphic solution. 
%           So, if you just want shorted executions, you need only look at the set of
%           homomorphic solutions.  (some symbol \mathcal{H}((W, \Vgoal)) might be useful to define the set, also in destructiveness.)



% The following is an interesting variation which we think is true,
% but likely requires space to define a notion of covering, which we 
% cannot afford here.
%
% The intention had been to remove the requirement that (P, A) solve some
% other planning problem, but other definitions are needed to do that.
% So, that requirement has been kept, but the second condition has been
% placed on vertices.
%
% IJRR: get this more general version written up.
%\begin{lemma}[self-solving plans (generalization)]
%  Suppose $P$ is
%  a p-graph with state set \mbox{$A \subseteq V(P)$}, such that plan $(P, A)$
%  solves some planning problem $(Q, G)$. 
%  When every vertex in $P$ appears
%  in some joint execution, we say that $(Q, G)$ {\em covers} $(P, A)$.
%  In such cases, $(P,A)$ is also a planning problem and, moreover, $(P,A)$ solves $(P,A)$.
%\end{lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commented out because subplans we never used for anything 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{theorem}\label{thm:subplan-destructive}
%  Suppose two plans $(P,\Pterm)$ and $(R,\Rterm)$ both solve a planning problem
%  $(G,\Vgoal)$, and that $(P,\Pterm)$ is a subplan of $(R,\Rterm)$.
%  If a map $h$ is destructive on $(P,\Pterm)$ for $(G,\Vgoal)$,
%  then $h$ is also destructive on $(R,\Rterm)$ for $(G,\Vgoal)$.
%  %
%  %  (P, \Pterm)<-------(subplan)-------(R, \Rterm)
%  %       |                                     | 
%  %       +--(solves)-->(G, \Vgoal)<--(solves)--+
%  % 
%\end{theorem}
%\begin{proofsketch}
%  The fact that $h$ is destructive on $(P,\Pterm)$ for $(G,\Vgoal)$ implies
%  that $(h(P),\Pterm)$ does not solve $(h(G),\Vgoal)$.  This means that at
%  least one of the four conditions in Definition~\ref{def:solves} is violated.
%  We show that in each of these four cases, $(h(R),\Rterm)$ does not solve
%  $(h(G), \Vgoal)$.
%  \begin{enumerate}
%    \item If $h(P)$ is not finite on $h(G)$, then for any $k$, there exists a
%    joint-execution of length greater than $k$ on $h(P)$ and $h(G)$.  This
%    execution is also a joint-execution on $h(R)$ and $h(G)$.
%
%    \item The case in which $h(P)$ not safe on $h(G)$ cannot occur, due to
%    Lemma~\ref{lem:map-safe}.
%
%    \item If $h(P)$ and $h(G)$ have some joint-execution $\eseq$ that is not a
%    prefix of an execution that reaches $\Pterm$, all joint-executions formed
%    by attaching some (possibly empty) suffix to $\eseq$ end outside of $\Pterm$.  In $\Rterm$,
%    both $\eseq$ and those non-goal-reaching suffixes remain as executions.
%    Treating $\eseq$ together with any such suffix as an execution not reaching the goal,
%    shows that $h(R)$ does not solve $h(G)$.
%    % This is subtle, because we need to argue that the map cannot create a
%    % *new* way to get to a goal.  I don't think this will happen --- the only
%    % thing that label maps can create is confusion --- but it seems nontrivial
%    % to write.  The idea is that, even if a path is created to reach a goal,
%    % there will still be some other path, not reaching the goal, that might be
%    % taken, and the execution that takes that path will fail.
%
%    \item If $h(P)$ and $h(G)$ have a joint-execution that reaches $\Pterm$,
%    but not $\Vgoal$.  This execution is also a joint-execution on $h(R)$ and
%    $h(G)$, and since we know that $\Pterm = \Rterm$, it also reaches a
%    termination state in $h(R)$, while reaching a non-goal state in $h(G)$.
%  \end{enumerate}
%  \vspace{-2em}
% \end{proofsketch}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  %%% ********** Here's the reasoning that led us to require \Pterm = \Rterm in
  %%% ********** the definition of subplan.
  %%% \begin{enumerate}
  %%%   \item If $h(P)$ is not finite on $h(G)$, then for any $k$, there exists a
  %%%   joint-execution of length greater than $k$ on $h(P)$ and $h(G)$.  This
  %%%   execution is also a joint-execution on $h(R)$ and $h(G)$.
%
  %%%   PROBLEM: none
%
  %%%   \item If $h(P)$ not safe on $h(G)$, then there exists some joint execution
  %%%   on $h(P)$ and $h(G)$, ending at state $v$ in $h(P)$ and state $w$ in
  %%%   $h(G)$, for which $v$ is missing an observation or $w$ is missing an
  %%%   action.
%
  %%%   PROBLEM: $h(R)$ might have this missing event.
%
  %%%   SOLUTION?: Is safety preserved by label maps?
%
  %%%   \item If $h(P)$ and $h(G)$ have some joint-execution that is not a prefix
  %%%   of an execution that reaches $\Pterm$.
%
  %%%   PROBLEM: This execution may be a prefix of something that DOES reach $\Rterm$.
%
  %%%   SOLUTION?: Change the definition of subplan.  Require $\Pterm = \Rterm$.
  %%%   (Or, strangely, $\Rterm \subseteq \Pterm$?)
%
  %%%   \item If $h(P)$ and $h(G$ have a joint-execution that reaches $\Pterm$, but
  %%%   not $\Vgoal$.  This execution is also a joint-execution on $h(R)$ and
  %%%   $h(G)$, and since we know that $\Pterm \subseteq \Rterm$, it also reaches a
  %%%   termination state in $h(R)$, while reaching a non-goal state in $h(G)$.
%
  %%%   PROBLEM: none (unless we change the definition of subplan as described above.)
%
  %%%   SOLUTION: Require $\Pterm = \Rterm$.
%
  %%% \end{enumerate}
%
%%% ********** And another, even earlier attempt at the proof:
%\begin{proofsketch}
%%If $(R,\Rterm)$ is a solution to $(G,\Vgoal)$ with $(P,\Pterm)$ a subplan of $(R,\Rterm)$, then as $(h(P),\Pterm)$
%If $(h(P),\Pterm)$ does not solve $(h(G),\Vgoal)$ it is because lacks one of:
%\begin{description}
%\item []\emph{finiteness:} any unending execution on $(h(P),\Pterm)$ can be traced on $(h(R),\Rterm)$ too, since the former is a subplan of the latter.
%\item []\emph{action safety:} if $(h(P),\Pterm)$ has some execution that involving execution of an action not in $(h(G),\Vgoal)$, then $(h(R),\Rterm)$ has the same execution too.
%\item []\emph{observation safety:} 
%%\item \emph{non-achievement (plan-sink):}  any execution on $(h(P),\Pterm)$ arriving at a sink not in $\Pterm$, will arr
%%\item \emph{non-achievement (problem-sink):}  any joint-execution on $(h(P),\Pterm)$ and $(h(G),\Vgoal)$ arrives at a sink on $(h(P),\Pterm)$ , with 
%%\item \emph{false-achievement (sink):}  any joint-execution on $(h(P),\Pterm)$ and $(h(G),\Vgoal)$ arriving at two sinks, with 
%\end{description}
%% I was tempted to say `success' instead of `non-achievement'
%\end{proofsketch}
%


% Thus, one might approach the problem of determining that a label map is
% strongly destructive by constructing the `extensive plan' $(P, \Pterm)$,
% presumably from some representative set of homomorphic solutions, perform
% language preserving operations (e.g., state-determined expansion, (exact)
% reduction) and then check for whether the map is destructive on that plan.


